Real-Time Neural Light Field on Mobile Devices

Recent efforts in Neural Rendering Fields (NeRF) have shown impressive results on novel view synthesis by utilizing implicit neural representation to represent 3D scenes. Due to the process of volumetric rendering, the inference speed for NeRF is extremely slow, limiting the application scenarios of utilizing NeRF on resource-constrained hardware, such as mobile devices. Many works have been conducted to reduce the latency of running NeRF models. However, most of them still require high-end GPU for acceleration or extra storage memory, which is all unavailable on mobile devices. Another emerging direction utilizes the neural light field (NeLF) for speedup, as only one forward pass is performed on a ray to predict the pixel color. Nevertheless, to reach a similar rendering quality as NeRF, the network in NeLF is designed with intensive computation, which is not mobile-friendly. In this work, we propose an efficient network that runs in real-time on mobile devices for neural rendering. We follow the setting of NeLF to train our network. Unlike existing works, we introduce a novel network architecture that runs efficiently on mobile devices with low latency and small size, i.e., saving $15\times \sim 24\times$ storage compared with MobileNeRF. Our model achieves high-resolution generation while maintaining real-time inference for both synthetic and real-world scenes on mobile devices, e.g., $18.04$ms (iPhone 13) for rendering one $1008\times756$ image of real 3D scenes. Additionally, we achieve similar image quality as NeRF and better quality than MobileNeRF (PSNR $26.15$ vs. $25.91$ on the real-world forward-facing dataset).

==> figs/4_limitation.tex <==
\begin{figure}[h]
  \dummyfig{Dummy Figure Label} 
%   \includegraphics[width=1.0\textwidth]{figs/foo}  
  \caption{\todo{limitation}}
  \label{fig:limitation}
\end{figure}

==> figs/5_latency.tex <==
\begin{figure}[h]
  \dummyfig{Dummy Figure Label} 
%   \includegraphics[width=1.0\textwidth]{figs/foo}  
  \caption{latency}
  \label{fig:latency}
\end{figure}

==> section/1_intro.tex <==
\section{Introduction}
\input{figs/0_teaser}

Recent studies on learning 3D scenes from a collection of 2D images have shown remarkable progress by leveraging implicit neural representation~\cite{park2019deepsdf,mescheder2019occupancy,chen2019learning,lombardi2019neural}. Among them, Neural Radiance Field (NeRF)~\cite{nerf} and its following works~\cite{mip-nerf,nerf-in-the-wild} demonstrate high-quality rendering for novel views. Specifically, a Multi-Layer Perceptron (MLP) is learned to estimate the radiance and density for the given coordinates of 3D points and view direction, which are used for view-dependent synthesis via volumetric rendering.




However, the impressive image quality of NeRF is at the cost of slow rendering speed. To estimate the color of one pixel, hundreds of points are sampled along the ray to integrate the radiance. Unable to run in real-time limits the applicable scenario of NeRF for real-world applications, such as Augmentation Reality, on resource-constrained hardware like mobile devices. 
Many efforts have been conducted to reduce the inference time of NeRF~\cite{kilonerf,plenoctrees,plenoxels,instant-ngp}. Nevertheless, they still require high-end GPUs with CUDA access for optimization that are unavailable on mobile devices.  
The most recent work of MobileNeRF~\cite{mobilenerf} shows the possibility of deploying the NeRF model on mobile devices by storing the calculated surface textures. Albeit the acceleration is promising, the method requires extra storage for saving textures, which is even more challenging for real-world scenes where complex polygons are estimated to model geometry. For example, on the face-forwarding LLFF dataset~\cite{nerf}, the memory per scene is $201.5$MB for MobileNeRF, $\todo{xxx} \times$ larger than NeRF ($\todo{xxx}$MB). 


On the other hand, Neural Light Field (NeLF) directly maps the given ray origins and view directions of a scene into the RGB color by only performing the network forward once per ray, resulting more favorable rendering speed than NeRF~\cite{levoy1996light,attal2022learning,liu2022neulf}. 
Due to the training difficulty of NeLF for high-fidelity rendering, Wang \emph{et al.}~\cite{r2l} introduce R2L - an $88$ layer of MLP with the residual connection that is trained via data distillation through utilizing a pre-trained NeRF as the teacher model. Although the deep MLP achieves better rendering results than NeRF with around $30\times$ acceleration, running it on mobile devices is still unable to perform real-time inference, \emph{i.e.,} $3$ seconds per image on iPhone 13 even for low resolution as $200\times200$.

In this work, we propose \modelname, a real-time neural rendering model on mobile devices trained via the similar data distillation pipeline of R2L~\cite{r2l}. Instead of using MLP-based networks that are applied by most works on implicit neural representation, we show that, a well-designed \emph{convolutional} (CONV)-based network for the neural light field can achieve real-time inference on mobile devices with a similar rendering quality as NeRF. In particular, we first revisit the network design choices of R2L and use the $1\times1$ CONV layer as a backbone. Second, we propose to gradually upsample the output from the backbone to a higher resolution, \emph{i.e.,} $800\times800$, rather than directly predicting high-resolution outputs from the backbone.  Overall, \modelname~favors several advantages over existing works:
\begin{itemize}[leftmargin=1em]
\setlength\itemsep{-0.5em}
    \item \modelname~achieves real-time inference speed  on mobile devices (Tab.~\ref{table:speed}) with better rendering quality, \emph{e.g.}, PSNR, than MobileNeRF on synthetic and real-world datasets (Tab.~\ref{table:quantitative}).
    \item \modelname~stores a scene by only using one neural network, dramatically reduces  ${15.2\times \sim  24.3\times}$ disk storage than MobileNeRF.
    \item The fast inference speed of \modelname~opens the door for us to leverage neural rendering to build real-world applications, such as virtual try-on, where the real-time interaction between devices and users is possible (Fig.~\ref{fig:teaser}).
\end{itemize}



==> tabs/latency.tex <==

\begin{table}[]
\begin{center}
\caption{
\textbf{Analysis of the spatial size of the input, usage of teacher model, and ray presentation}. Besides image quality metrics, we show the number of parameters for each model and the latency when running on iPhone 13. }\label{table:latency}
% \vspace{-3mm}
\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lccccc}
\toprule
 & Params & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Latency$\downarrow$ \\
\midrule
{$50\times50$ - NeRF Teacher} &3.9M &30.40 & 0.9965 & 0.0686 &  13.04 \\
{$100\times100$ - NeRF Teacher} &3.9M & 30.65 &0.9966  &0.0668  & 26.21 \\
{$200\times200$ - NeRF Teacher} &3.9M & - &- &-  &  73.76 \\
{$800\times800$ - w/o SR} &3.9M & - & - & - &  Error \\ \hdashline
{$100\times100$ - MipNeRF Teacher} & 3.9M&  30.83 & 0.0997 & 0.0564 & 26.21 \\ 
{$100\times100$ - MipNeRF Teacher, $K16$, $L10$} &4.1M & 30.90 &0.9968  & 0.0583  & 31.05  \\ 
$100\times100$ - MipNeRF Teacher, $K16$, $L10$, D100 &6.8M & 31.37 & 0.9972 &0.0470  & 44.52 \\
\bottomrule
\end{tabular}
}
\end{center}
% \vspace{-4mm}
\end{table}

